Efficient approximation schemes for uniform-cost clustering problems in planar graphs

We consider the $k$-Median problem on planar graphs: given an edge-weighted planar graph $G$, a set of clients $C \subseteq V(G)$, a set of facilities $F \subseteq V(G)$, and an integer parameter $k$, the task is to find a set of at most $k$ facilities whose opening minimizes the total connection cost of clients, where each client contributes to the cost with the distance to the closest open facility. We give two new approximation schemes for this problem: -- FPT Approximation Scheme: for any $\epsilon>0$, in time $2^{O(k\epsilon^{-3}\log (k\epsilon^{-1}))}\cdot n^{O(1)}$ we can compute a solution that (1) has connection cost at most $(1+\epsilon)$ times the optimum, with high probability. -- Efficient Bicriteria Approximation Scheme: for any $\epsilon>0$, in time $2^{O(\epsilon^{-5}\log (\epsilon^{-1}))}\cdot n^{O(1)}$ we can compute a set of at most $(1+\epsilon)k$ facilities (2) whose opening yields connection cost at most $(1+\epsilon)$ times the optimum connection cost for opening at most $k$ facilities, with high probability. As a direct corollary of the second result we obtain an EPTAS for the Uniform Facility Location on planar graphs, with same running time. Our main technical tool is a new construction of a "coreset for facilities" for $k$-Median in planar graphs: we show that in polynomial time one can compute a subset of facilities $F_0\subseteq F$ of size $k\cdot (\log n/\epsilon)^{O(\epsilon^{-3})}$ with a guarantee that there is a $(1+\epsilon)$-approximate solution contained in $F_0$.

==> conclusions.tex <==
\section{Conclusions}\label{sec:conclusions}

In this work we have advanced the understanding of approximability of {\sc{(Uniform) Facility Location}} and {\sc{$k$-Median}} on planar graphs by giving several approximation schemes.
For {\sc{Facility Location}} we gave the first QPTAS and for {\sc{Uniform Facility Location}} we gave the first EPTAS, improving upon the PTAS of Cohen-Addad et al.~\cite{Cohen-Addad:2018}.
For {\sc{$k$-Median}} we gave an FPT approximation scheme and a bicriteria EPTAS.

The main question that remains open is whether the QPTAS for {\sc{Facility Location}} can be improved to a PTAS.
The running time provided in Section~\ref{sec:nufl} is $2^{\Oh(\eps^{-3}\log^4 n)}$. These four $\log n$ factors can be traced as follows:
\begin{enumerate}
\item The first $\log n$ factor comes from the resolution width of every ring $W_k$, which is $(K+1)L$. While $K=\Oh(\eps^{-1})$, we have $L=\Oh(\log (n/\eps))$. 
The necessity of having factor $\log n$ in the width of the isolation layer can be traced to the use of Lemma~\ref{lem:voronoi-logn-radius} within the proof of the isolation property, Lemma~\ref{lem:nufl:isolation}.
\item The second $\log n$ factor comes from the choice of $\delta=\Oh(\eps/\log n)$. Namely, when solving the generalized problem by recursion,
we need to use an accuracy parameter smaller by factor $\Oh(\log n)$ to make up for the errors stacking up through $\Oh(\log n)$ recursion levels.
\item The third $\log n$ factor is introduced in the recursion, when we guess, for every portal $\pi$, the facilities $\gamma_1(\pi)$ and $\gamma_2(\pi)$ serving this portal.
There are $(n+1)$ options to choose each of them, yielding a $\log n$ factor in the exponent.
\item The fourth $\log n$ factor is introduced by the recursion itself: a recursion of branching $d$ and depth $\Oh(\log n)$ has $d^{\Oh(\log n)}$ recursive calls in total.
\end{enumerate}
We now sketch how using some more involved technical reasoning two of these factors, namely the third and the fourth, can be shaved off.
In the description provided in Section~\ref{sec:nufl} we decided to present the algorithm with suboptimal running time, in order not to obfuscate the main ideas with technical details of secondary importance.

The fourth $\log n$ factor is actually easy to shave off if we replace Divide\&Conquer with dynamic programming.
Namely, observe that the structure of the recursion tree --- consecutive balanced separators used, is independent of the guesses made throughout the recursion.
Therefore, we may first compute a hierarchical decomposition of the client set of depth $\Oh(\log n)$, and to each node of this decomposition assign an instance of the 


Thus, in order to improve the QPTAS to a PTAS, there is only one more $\log n$ factor to shave of.
We believe that the second $\log n$ factor would be very difficult to shave off. 
The phenomenon of error stacking throughout $\Oh(\log n)$ levels of recursion is notorious in the design of approximation schemes, 
see the recent line of work on QPTASes for geometric packing and covering problems~\cite{AdamaszekW13,AdamaszekW14,ChuzhoyE16,Har-Peled14,PilipczukLW18},
and so far there is no good way known of circumventing the issue.
Shaving off the first $\log n$ factor seems far more plausible, and the question boils down to the following: can one somehow 
use isolation of resolution width $L=\textrm{poly}(\eps^{-1})$ instead of $L=\Oh(\log (n/\eps))$
and achieve the necessary isolation property, i.e., an analogue of Lemma~\ref{lem:nufl:isolation}?



